Detecting Redundant CSS Rules in HTML5 Applications: A Tree-Rewriting Approach

HTML5 applications normally have a large set of CSS (Cascading Style Sheets) rules for data display. Each CSS rule consists of a node selector (given in an XPath-like query language) and a declaration block (assigning values to selected nodes' display attributes). As web applications evolve, maintaining CSS files can easily become problematic. Some CSS rules will be replaced by new ones, but these obsolete (hence redundant) CSS rules often remain in the applications. Not only does this "bloat" the applications, but it also significantly increases web browsers' processing time. Most works on detecting redundant CSS rules in HTML5 applications do not consider the dynamic behaviors of HTML5 (specified in JavaScript); in fact, the only proposed method that takes these into account is dynamic analysis (a.k.a. testing), which cannot soundly prove redundancy of CSS rules. In this paper, we introduce an abstraction of HTML5 applications based on monotonic tree-rewriting and study its "redundancy problem". We establish the precise complexity of the problem and various subproblems of practical importance (ranging from P to EXP). In particular, our algorithm relies on an efficient reduction to an analysis of symbolic pushdown systems (for which highly optimised solvers are available), which yields a fast method for checking redundancy in practice. We implemented our algorithm and demonstrated its efficacy in detecting redundant CSS rules in HTML5 applications.

==> applications.tex <==
% !TEX root = main-LICS14.tex

\emph{Cascading style sheets} (CSS) are a language for describing the look and formatting of an XML document or a document written in a markup language. Designed to enable the separation of document content from document presentation, CSS includes elements such as layout, colour and font. Abstractly, if one models web documents as unranked trees then a CSS is just a list of rules, each rule consisting of a guard (or selector) and a tree operation.

As a web application evolves, rules that are never used, and hence redundant, can accumulate over time. A recent empirical study of several open-source and industrial web applications \cite{MesbahM12} shows that 60\% of selectors were redundant; furthermore visual layout consumes 40-70\% of the average processing time of a web page. Thus a pertinent question for web development and maintenance is whether a given CSS rule is redundant. See also \cite{GenevesLQ12}.

\subsection{Contributions of the paper}

\subsection{Related work}



==> counter-examples.tex <==


\newcommand\witnesstree{\mathrm{Tree}}
\newcommand\getpdswitness{\mathrm{Witness}}

\section{Witness Generation}

The proofs of correctness of our fixpoint computation
(Lemma~\ref{lm:reduce-class-adding}) and sPDS reduction
(Lemma~\ref{lm:spds-correctness}) give us directly a witness generation
algorithm.  We extract this algorithm here for clarity.

For a rewrite system $\trs$ over $\treelabels$-trees, a finite nonempty set $S$
of guards over $\treelabels$, and an initial $\treelabels$-labeled tree
$\tree_0$, suppose the guard $g \in S$ is matched in $\post_{\trs}^*(\tree_0)$.
We show how to construct a sequence $(v_1, \sigma_1, \tree_1), \ldots, (v_n,
\sigma_n, \tree_n)$ of pairs of nodes and rules in $\trs$ that witnesses a
matching of $g$ in $\post_{\trs}^*(\tree_0)$.  That is, for all $1 \leq i \leq
n$ we have
\[
    \tree_{i-1} \to_{\sigma_i} \tree_i
\]
with $\tree_i = (\treedomain_i, \treelabeling_i)$, $v_i \in \treedomain_i$ and
in particular, $\sigma_i$ is applied at node $v_i$.

As per Section~\ref{sec:upper} we can assume that $g \in \CLASS'$ and that $g
\in \treelabeling_n(\epsilon)$.  Due to monotonicity, it is in fact possible to
construct, alongside the fixpoint construction, a single witness that acts as a
counter example for all $c \in \CLASS$ matched at the root node.

We introduce some notation for convenience.  For any sequence $W \in (\N^\ast
\times \trs \times \trees(\treelabels))^\ast$ let
\[
    \witnesstree(W) =
    \begin{cases}
        \tree_0 & W = \epsilon \\

        \tree & W = W' (v, \sigma, \tree) \ .
    \end{cases}
\]
Additionally, we write $\tree[v \mapsto A]$ to denote the tree obtained by
extending the label of node $v$ in $\tree$ with the classes in $A$, or adding
the node if it does not already exist.  That is, when $\tree = (\treedomain,
\treelabeling)$, we have $\tree[v \mapsto A] = (\treedomain', \treelabeling')$
where $\treedomain' = \treedomain \cup \{v\}$ and for all $v' \in \treedomain'$,
\[
    \treelabeling'(v') =
    \begin{cases}
        \treelabeling(v') \cup A & v' = v \in \treedomain \\

        A & v' = v \notin \treedomain \\

        \treelabeling(v') & v' \neq v \ .
    \end{cases}
\]


We recall the fixpoint computation while simultaneously constructing the witness
$W$.  Initially, let $\tree = (\treedomain,\treelabeling) := \tree_0$ and
\[
    W = \epsilon \ .
\]
At each step, we apply of the following rules.
\begin{itemize}
    \item
        If $\sigma = (g,\addclass{B})$ is applicable at a node $v \in
        \treedomain_0$, then $\treelabeling(v) := \treelabeling(v) \cup B$.
        Furthermore, let $\tree' = \witnesstree(W)[v \mapsto B]$ and $W := W (v,
        \sigma, \tree')$.

    \item
        Take $v \in \treedomain$, $c \in \CLASS \setminus \treelabeling(v)$, and
        $\tree_v := (\epsilon,\treelabeling_v)$ with $\treelabeling_v(\epsilon)
        = \treelabeling(v)$. Define $f: (\{\Root\}\cup\CLASS) \to \{0,1\}$ with
        $f(\Root)=1\LRA v = \epsilon$ and, if $f(\Root) = 0$ and $u$ is the
        parent of $v$, then $f(a)=1 \LRA a\in \treelabeling(u)$. Then, if the
        class-adding problem has positive answer on input $\langle
        \tree_v,f,c,\trs\rangle$, then $\treelabeling(v) := \treelabeling(v)
        \cup \{c\}$.  Furthermore, let $\rho$ be a sequence of pushdown
        operations witnessing the positive solution of the bit-toggling problem
        obtained from the class-adding problem.  We set $W := \getpdswitness(v,
        \rho, W)$ and $\getpdswitness$ is defined below.  Note, witness
        generation algorithms for pushdown systems are well-known
        (E.g.~\cite{schwoon-thesis}).

\end{itemize}

The function $\getpdswitness(v, \rho, W)$ extends W with a sequence of rule
applications and trees from a given node and run of a pushdown system
constructed to solve the bit-toggling problem by the reduction in the proof of
Lemma~\ref{lm:reduce}.  First, observe, in this reduction, each rule of the sPDS
either pops the stack or is directly derived from a rule in $\trs$.  We define
$\getpdswitness$ recursively in Algorithm~\ref{alg:getpdswitness}, described
below.

\begin{algorithm}
    \caption{\label{alg:getpdswitness}$\getpdswitness(v, \rho, W)$}
    \begin{algorithmic}
        \If {$\rho = \epsilon$}
            \Return {$W$}
        \Else
            \State {Let $(i, \varphi) \rho' = \rho$}
            \State {Let $\tree = (\treedomain, \treelabeling) = \witnesstree(w)$}
            \If {$i = 0$}
                \State {\Return {$(W, \rho')$}}
            \ElsIf {$i = 1$}
                \State {Let $\sigma = (g, \addclass{B})$ derive $(i, \varphi)$}
                \State {Let $W' = W (v, \sigma, \tree[v \mapsto B])$}
                \State {\Return {$\getpdswitness(v, \rho', W')$}}
            \Else
                \State {Let $\sigma = (A, \addchild{B})$ derive $(i, \varphi)$}
                \State {Let $j$ be the smallest $j$ such that $vj \notin \treedomain$}
                \State {Let $W' = W (v, \sigma, \tree[vj \mapsto B])$}
                \State {Let $(W'', \rho'') = \getpdswitness(vj, \rho', W')$}
                \State {\Return {$\getpdswitness(v, \rho'', W'')$}}
            \EndIf
        \EndIf
    \end{algorithmic}
\end{algorithm}

The algorithm in Algorithm~\ref{alg:getpdswitness} takes a sequence
of pushdown rules and extracts the corresponding run of the tree rewrite
system.  It takes as arguments a sequence of pushdown operations $\rho$, the
node $v$ of the tree the first rule of $\rho$ is applied to, and $W$ the
witness generated so far.

To begin, it takes the first pushdown rule of $\rho$, and last tree $\tree$ of
$W$ and then case splits on the rule.
\begin{itemize}
    \item
        If it is a pop, then we are done with the portion of $\rho$ that
        operates on $v$, and so return the witness generated and the remaining
        rules to process.

    \item
        If it is a rule that does not change the stack height, then we obtain
        the $\addclass{B}$ rule of the tree rewrite system it came from, and
        extend the witness by applying this rule to $\tree$.  We then use
        tail-recursion to obtain the remainder of the witness.

    \item
        If is is a push rule, then it was derived from an $\addchild{B}$ rule
        and begins a sequence of operations applied to the new child.  Hence,
        we add a new child to $\tree$ and recursively call the algorithm to
        process the sequence of rules applied to this new node.  Once this call
        returns, we continue processing the rules remaining to be applied to
        the current node via tail-recursion.
\end{itemize}



==> decidability.tex <==
% !TEX root = main-LICS14.tex
\section{Decidability and Complexity}
%\lochanged{In this section, we study a more restricted class of monotonic tree rewrite systems with tree operations restricted to $\addchild{X}$ and $\addclass{X}$ only.}


To prove $\W[1]$-hardness, we reduce from the short acceptance problem of
nondeterministic Turing machines.
%: given a triple $\langle \TM,w,k \rangle$,
%where $\TM$ is an NTM, $w \in \{0,1\}^*$ is an input word, and $k$ is positive
%integer represented in unary, decide whether $\TM$ accepts $w$ in $k$
%steps.
The input to the problem is $\langle \TM,w;k\rangle$, where $\TM$ is an NTM,
$w$ is an input word for $\TM$, and $k \in \N$ given in unary.
Suppose that $\TM =
(\oalphabet,\talphabet,\blank,\controls,\pdsrules,q_0,q_{acc})$,
where $\oalphabet = \{0,1\}$ is the input alphabet, $\talphabet =
\{0,1,\blank\}$ is the tape alphabet, $\blank$ is the blank symbol, $\controls$
is the set of control states, $\pdsrules \subseteq (\controls \times \talphabet)
\times (\controls \times \talphabet \times \{L,R\})$ is the transition relation
($L$/$R$ signify go to left/right), $q_0 \in \controls$ is the initial
state, and $q_{acc}$ is the accepting state. Each configuration of $\TM$ on $w$
of length $k$ can be represented as a word
\[
    (0,a_0,c_0)(1,a_1,c_1)\cdots (k,a_k,c_k)
\]
where $a_i \in \talphabet$ for each $i \in [0,k]$, and for some $j \in [0,k]$
we have $c_j \in \controls$ and for all $r \neq j$ it is the case that
$c_j = \star$. Note that this is a word (of a certain kind) over $\Omega := \Omega_k := [0,k] \times \talphabet
\times (\controls \cup \{\star\})$. In the sequel, we denote by
$\CONF_k$ the set of all configurations of $\TM$ of length $k$.
Suppose that $w = a_1\cdots a_n$. If
$n < k$, we append some blank symbols at the end of $w$ and assume that
$|w| \geq k$. The initial configuration will be
$I_0(w) := (0,\blank,q_0)(1,a_1,\star)\cdots (k,a_k,\star)$. [Notice that
if $n > k$, then some part of the inputs will be irrelevant.]
In the following, we will append the symbol $(-1,\blank,\star)$ (resp.
$(k+1,\blank,\star)$) before the start (resp. after the end) of $\TM$
configurations to aid our definitions. Therefore, define
$\Omega_e := \Omega_{k,e} := [-1,k+1] \times \talphabet
\times (\controls \cup \{\star\})$.

%\lo{Why go beyond ${[0, k]}$?}

We now construct a tree-rewrite system $\pds$ to simulate $\TM$. First off,
for each $\pdsrules$-rule $\sigma$,
define a relation $R_\sigma \subseteq \Omega_e^4$ such that
$(\vecV_1,\vecV_2,\vecV_3,
\vecW) \in R$ iff a configuration $C_2 = \vecU_{-1} \cdots
\vecU_{k+1}$ of $\TM$, where $\vecU_{i+1} = \vecW$ for some $i$, can be
reached in one step using $\sigma$ from another
configuration
$C_1 = \vecU_{-1}' \cdots \vecU_{k+1}'$, where $\vecU_i'\vecU_{i+1}'\vecU_{i+2}' =
\vecV_1\vecV_2\vecV_3$. Let $R = \bigcup_{\sigma\in\pdsrules} R_\sigma$.
In this case, we say that rule $\sigma$ is a witness
for the tuple $(\vecV_1,\vecV_2,\vecV_3,\vecW)$. Notice that, given a rule
$\sigma$ of $\pds$ and $\vecV_1,\vecV_2,\vecV_3$, there exists
\emph{at most one} $\vecW$ such that $(\vecV_1,\vecV_2,\vecV_3,\vecW)
\in R$ and is witnessed by $\sigma$. In addition,
it is easy to see that checking whether
$(\vecV_1,\vecV_2,\vecV_3,\vecW) \in R$ can be done in polynomial time
(independent of $k$) since this is a simple local check of $\TM$
rules.

The rewrite system $\pds$ works over trees of labels $\Xi = \Omega_e
\cup \pdsrules$. \lo{As defined, labels must be elements of a power set $\treelabels = 2^\CLASS$.} The initial tree is a tree with a single node labeled by
$I_0(w)$. We add the following rules to $\pds$:
\begin{enumerate}
\item For each $\sigma \in \pdsrules$, we add $(\top,\addchild{\sigma})$
    to $\pds$.
\item For each $(\vecV_{i-1},\vecV_i,\vecV_{i+1},\vecW) \in R$ witnessed by
    $\sigma \in \pdsrules$, for $i \in [0,k]$,
    we add $(\{\sigma\}\langle \uparrow
    \rangle\{\vecV_{i-1},\vecV_i,\vecV_{i+1}\},
    \addclass{\vecW})$ to $\pds$.
\item For each $\sigma \in \pdsrules$, we add
    $(\{\sigma\},\addclass{(-1,\blank,\star)})$ and
    $(\{\sigma\},\addclass{(k+1,\blank,\star)})$ to
    $\pds$.
\end{enumerate}
Rule 1 first guesses the rule $\sigma$ to be applied to obtain the next
configuration $C_2$ of the NTM $\TM$. This rule is added as a class in the
child $v$ of the current node $u$ containing the current configuration $C_1$.
Rule 3 is then applied to obtain the left and right delimiter. After that,
configuration $C_2$ is written down in node $v$ by applying Rule 2 for $k$
times. In particular, the system will look up the rule $\sigma$ that was
guessed before and the content of the parent node $u$ (i.e. $C_1$). If we
let $S = [0,k] \times \talphabet \times \{q_{acc}\}$, then $S$ is not
$k$-redundant iff $\TM$ accepts $w$ within $k$ steps. Notice that this is
an fpt-preserving reduction. In particular, it runs in time $O(\poly(k) \times
\poly(n))$.

%\subsubsection{Proof of $\P$ algorithm}
\subsubsection{Proof of solvability in $\P$}


We now provide an algorithm for the $k$-redundancy problem that runs in time
$O(n^k)$. The input to the algorithm is a rewrite system $\trs$ over
$\treelabels$-labeled trees, a guard database $S$ over $\trees(\treelabels)$,
and an initial $\treelabels$-labeled tree $\tree_0 =
(\treedomain_0,\treelabeling_0)$. Our algorithm will compute a tree
$\tree_F = (\treedomain_F,\treelabeling_F)$ such that
$\tree_F \in \post_\trs^*(\tree_0)$ and, for all tree $\tree \in
\post_\trs^*(\tree_0)$, we have $\tree \trleq \tree_F$. By Lemma \ref{lm:trleq},
if a guard $g \in S$ is matched in some $\tree \in \post_\trs^*(\tree_0)$,
then $g$ is matched in $\tree_F$. The converse also holds since
$\tree_F \in \post_\trs^*(\tree_0)$. Furthermore, we shall see that
$\tree_F$ is of height at most $k$, each of whose nodes has at most
$\sizeof{\tree_0}+|\trs|$ children (and so of size at most
$O((\sizeof{\tree_0}+|\trs|)^k)$), and is computed in time
$O(|\treelabels| \times (\sizeof{\tree_0}+|\trs|)^k)$. Computing the rules
in $S$ that are matched in $\tree_F$ can be done in time linear in
$\sizeof{S} \times \sizeof{\tree_F}$ by a standard marking algorithm.


\newcommand\dom{\mathit{dom}}
\newcommand\calF{{\cal F}}
\newcommand\makeset[1]{\{#1\}}


The algorithm for computing $\tree_F$ works as follows.
\begin{description}
\item[(1)] Set $\tree = (\treedomain,\treelabeling) := \tree_0$;
\item[(2)] Set $W := \emptyset$;
\item[(3)] Add each pair $(v,\sigma)$ to $W$, where $v \in \treedomain$ and
    $\sigma \in \trs$ is a rule that is applicable at $v$ i.e.~$v, T \models g$ where $\sigma = (g, \chi)$ for some $\chi$; all pairs in $W$ are initially
    ``unmarked'';
\item[(4)] Repeat the following for each unmarked pair $(v,\sigma) \in W$
    with $\sigma = (g,\chi)$:
    \begin{description}
    \item[(a)] if $\chi = \addclass{X}$, then $\treelabeling(v) :=
        \treelabeling(v) \cup X$;
    \item[(b)] if $\chi = \addchild{X}$, $|v| < k - 1$, and
        $X \not\subseteq \treelabeling(v.i)$ for \emph{each} $v.i \in
        \treedomain$ child of $v$,
        % \lo{I think the preceding condition should be: $\forall i \in M_v \, . \, X \not\subseteq \treelabeling(v.i)$ where $M_v = \makeset{i \mid v.i \in \dom(\treelabeling)}$.}
        %\al{Spot on}
        then
        set $\treedomain := \treedomain \cup \{v.(i+1)\}$  where
        $i := \max\{ j \in \N : v.j \in \treedomain\} + 1$ (by convention,
        $\max\emptyset = 0$), and $\treelabeling(v.j) := X$;
    \item[(c)] Mark $(v,\sigma)$;
    \item[(d)] For each $(v,\sigma) \in (\treedomain \times
        \trs) \setminus W$ that is applicable, add $(v,\sigma)$ to
        $W$ unmarked;
    %\item[(e)] If \textbf{(d)} adds no new pair, then go to \textbf{(5)};
    \end{description}
\item[(5)] Output $\tree_F := \tree$;
\end{description}
\lo{This is a fixpoint construction. More on this shortly.}

\noindent
\textbf{Proof of Correctness.} We will show that $\tree \trleq \tree_F$
for each $\tree \in \post_\trs^*(\tree_0)$. The proof is by induction on
length $m$ of path from $\tree_0$ to $\tree$. We write $\tree_F =
(\treedomain_F,\treelabeling_F)$. The base case is when $m=0$,
in which case $\tree = \tree_0 = (\treedomain_0,\treelabeling_0)$. Since
our rewrite rules only add classes to nodes and add new nodes, it is
immediate that $\treedomain_0 \subseteq \treedomain_F$ and that
$\treelabeling_0(v) \subseteq \treelabeling_F(v)$ for each $v \in
\treedomain_0$. That is, $\tree_0 \trleq \tree_F$. We now proceed to the
inductive step and assume that $\tree = (\treedomain,\treelabeling) \trleq
\tree_F$ with a witnessing function $f: \treedomain \to \treedomain_F$.
Let $v \in \treedomain$ and $\sigma = (g,\chi)$ be a $\trs$-rule that is
applicable on the node $v$ of $\tree$. By Lemma \ref{lm:trleq}, it follows that
$f(v), \tree_F \models g$. Let us suppose that after applying $\sigma$ on
$v$, we obtain $\tree' := (\treedomain',\treelabeling')$.
We have two cases now:
\begin{enumerate}
\item $\chi = \addclass{X}$. In this case, $\treedomain' = \treedomain$,
$\treelabeling'(u) = \treelabeling(u)$ whenever $u \neq v$, and
$\treelabeling'(v) = \treelabeling(v) \cup X$. Since $\tree \trleq
\tree_F$, it follows that $\treelabeling(f v) \subseteq \treelabeling_F(v)$.
Since $f v,\tree_F \models g$, it follows that $(f v,\addclass{X})$ is marked in
$W$ (by the end of the computation of $\tree_F$).
This means that $X\subseteq \treelabeling_F(f v)$. Altogether,
$\tree' \trleq \tree_F$.
\item $\chi = \addchild{X}$ and $|v| < k-1$. In this case, $\treedomain' =
\treedomain
\cup \{ v.i \}$ for some $i \in \N$ with $v.i \notin \treedomain$,
$\treelabeling'(u) = \treelabeling(u)$ for each $u \in \treedomain$,
and $\treelabeling'(v.i) = X$. Since $\tree \trleq \tree_F$, it follows that
$v$ and $f v$ have the same levels in $\tree$ and $\tree_F$ respectively.
Also, since $v,\tree_F \models g$, it follows that $(f v,\addchild{X})$ is
marked in $W$ (by the end of the computation of $\tree_F$). This means that
a child $f(v).j$ was added to $\treedomain_F$ with $X \subseteq
\treelabeling_F(f(v).j)$. Hence, the extension of $f$ with $f(v.i) := f(v).j$
is a witness for $\tree' \trleq \tree_F$, as desired.
\end{enumerate}

\input{fixpoint-algorithm}


\noindent
\textbf{Running time analysis.} To be added


\input{pspace-lb-decidability.tex}
\input{pspace-ub-decidability.tex}


==> extensions.tex <==
\section{Extending the model}
\label{sec:extension}
Here, we briefly consider the extension of our current model to allow the
ability to remove classes. More precisely, we allow rewrite rules of the form
$\sigma = (g,\chi)$, where $g$ is a guard and $\chi = \removeclass{X}$ for some
$X \subseteq \CLASS$. The semantics is defined as follows. Given two trees
$\tree = (\treedomain,\treelabels)$ and $\tree' = (\treedomain',\treelabels')$,
we write $\tree \to_\sigma \tree'$ if (i) $\treedomain' = \treedomain$, (ii)
there exists a node $v \in \treedomain$ such that $v \models g$, and
(iii) $\treelabels'(v) = \treelabels(v) \setminus X$ and
$\treelabels(w) = \treelabels(w)$ for each $w \neq v$.
\begin{proposition}
The redundancy problem for $\trsclass$ is undecidable.
\end{proposition}

\begin{proof}
Reduction from the acceptance problem for a fixed (i.e. universal) Turing
machine $M = (\oalphabet,\talphabet,\blank,\controls,\pdsrules,q_0,q_{acc})$,
where $\oalphabet = \{0,1\}$ is an input alphabet, $\talphabet =
\{0,1,\blank\}$ is the tape alphabet, $\blank$ is the blank symbol, $\controls$
is the set of control states, $\pdsrules: (\controls \times \talphabet)
\to (\controls \times \talphabet \times \{L,R\})$ is the transition function
($L$/$R$ signify go to left/right), $q_0 \in \controls$ is the initial
state, and $q_{acc}$ is the accepting state. A configuration of $M$
is a word of the form $v(q,a)w$, where $v,w \in \oalphabet^*$, $a \in
\oalphabet$, and $q \in \controls$. Given an input word $w =
a_1\cdots a_n \in \oalphabet^*$, the initial configuration is
$I_0(w) = (q_0,\blank)a_1\cdots a_n$. An \defn{accepting} configuration is
of the form $(q_{acc},\blank)\blank^m$ for some $m \in \N$.
Given two configurations $C,C'$ of
$M$,
we write $C \entails C'$ to mean that $C'$ is a configuration
that proceeds $C$ according to the transition rule $\pdsrules$ (which is
defined in the standard way). The word $w$ is \defn{accepted} by $M$ if $I_0(w)
\entails^* C$ for some accepting configuration $C$.

We now show how to reduce this to the redundancy problem. Firstly, set
$\treelabels = \talphabet \cup (\controls \times \talphabet) \cup (\controls
\times \talphabet \times \{L,R\})$. The initial tree $\tree_0$ is set to
be $I_0(w)$. The set of guards is the singleton $\{(q_{acc},\blank)\}$, i.e.,
checking the existence of a node labeled $(q_{acc},\blank)$. We next define the
rewrite system $\trs$.

The crux is to simulate one transition step of $M$ by a number of intermediate
steps of
$\trs$. For example, we simulate the transition $00(q,1)1 \entails 0(q',0)01$
of $M$ by means of several $\trs$ steps $00(q,1)1 \to_\trs 00(q',0,L)1 \to_\trs
0(q',0)(q',0,L)1 \to_\trs 0(q',0)01$. More formally, ...
\qed
\end{proof}

\begin{theorem}
For every $k \in \N_{> 0}$, the $k$-redundancy problem for $\trsclass$
is complete for $(k-1)$-$\EXPSPACE$.
\end{theorem}
\al{I think we can simply just put a decidability result here via
embedding to well-structured transition systems and save this upper bound for
some other paper}


==> fixpoint-algorithm.tex <==
% !TEX root = main-LICS14.tex

\subsection*{Definition of $T_F$}
Let $T = (D_T, \treelabeling_T)$. Define an endofunction $F$ on $\trees_k(\treelabels)$ by $T \mapsto F(T) = (D_{F(T)}, \treelabeling_{F(T)})$ where $D_{F(T)} := D_T \cup \makeset{v . |M_v| \mid H_{v, T}}$ with $M_v := \makeset{i \mid v.i \in D_T}$ and 
\begin{align*}
H_{v, T} \, := \, &[v \in D_T, (g, \addchild{X}) \in \trs, \\ & v, T \models g, \forall i \in M_v . X \not\subseteq \treelabeling_T(v.i)].
\end{align*}
%$H_{v, T} := [v \in D_T, (g, \addclass{X}) \in \trs, v, T \models g, \forall i \in M_v . X \not\subseteq \treelabeling_T(v.i)]$. %Notice that $D_T$ and $\makeset{v . |M_v| \mid H_{v, T}}$ are disjoint. 
Note that $D_T$ and $\makeset{v . |M_v| \mid H_{v, T}}$ are disjoint sets. Let $v \in D_{F(T)}$. Define
\[
\treelabeling_{F(T)}(v) := 
\left\{
\begin{array}{ll}
\treelabeling_T(v) \cup \bigcup\makeset{X \mid L_{v, T}} & \hbox{if $v \in D_{T}$} 
\\
X & \hbox{if $v \in \makeset{u . |M_u| \mid H_{u, T}}$}
\end{array}
\right.	
\]
where $L_{v, T} = [v \in D_T, (g, \addclass{X}) \in \trs, v, T \models g]$. 

\lo{``$H$'' is for $\addchild{X}$ and ``$L$'' is for $\addclass{X}$.}
%If $v \in D_{T}$, define $\treelabeling_{F(T)}(v) := \treelabeling_T(v) \cup \bigcup\makeset{X \mid L_{v, T}}$ where $L_{v, T} = v \in D_T, (g, \addclass{X}) \in \trs, v, T \models g$. If $v = u . |M_u| \in \makeset{v . |M_v| \mid H_{v, T}}$ then define $\treelabeling_{F(T)}(u . |M_u|) := X$.

\begin{lemma}\label{lem:monotone}
$F$ is $\trleq$-monotone. 
\end{lemma}

\begin{proof}
Suppose $T \trleq T'$ via $f : D_T \to D_{T'}$. We shall prove $F(T) \trleq F(T')$ and define its witnessing function $f' : D_{F(T)} \to D_{F(T')}$ simultaneously. First we set $f' \restriction D_T := f$. Take $v \in D_{F(T)}$ such that $v \in D_T$. Thanks to Lemma~\ref{lem:preserve-vDash}, we have for every $g$, if $L_{v, T}$ then $L_{f'(v), T'}$. Hence 
\begin{align*}
\treelabeling_{F(T)}(v) & := \treelabeling_T(v) \cup \bigcup \makeset{X \mid L_{v, T}} \\
& \subseteq \treelabeling_{T'}(f'(v)) \cup \bigcup \makeset{X \mid L_{f'(v), T'}} \\
& = \treelabeling_{F(T')}(f'(v))
\end{align*}
as desired. Next take %$v \in D_{F(T)}$ such that 
$v = u . |M_u| \in \makeset{u . |M_u| \mid H_{u, T}}$. Two cases:
\begin{inparaitem}
\item[Case 1:] $\forall i \in M_{f(u)} . X \not\subseteq \treelabeling_{T'}(f(v).i)$. Then, by definition, %$f(u) . |M_u| \in D_{F(T')}$ and 
$\treelabeling_{F(T')}(f(u) . |M_{f(u)}|) = X$. Define $f'(u . |M_u|) := f(u) . |M_{f(u)}| = f'(u) . |M_{f'(u)}|$. Then $\treelabeling_{F(T)}(u.|M_u|) = X = \treelabeling_{F(T')}(f'(u.|M_u|))$ as desired. 
\item[Case 2:] $X \subseteq \treelabeling_{T'}(f(u) . i)$ for some $i \in M_u$. Set $f'(u . |M_u|) := f'(u) . i$. Then $\treelabeling_{F(T)}(u . |M_u|) = X \subseteq \treelabeling_{F(T')}(f'(u . |M_u|))$.
\end{inparaitem}
\end{proof}

Since $F$ is monotone, define $T_F$ to be the least upper bound of $\makeset{F^i(T_0) \mid i \geq 0}$, which is well-defined as the set has an upper bound.

%\lo{It seems that Knaster-Tarski Theorem does not apply here: an arbitrary monotone function may not have a fixpoint. To be clarified.}
%Let $T = (\dom(\treelabeling), \treelabeling)$. Define $F (\treelabeling) := \treelabeling \cup L(\treelabeling) \cup H(\treelabeling)$ where 
% \begin{align*}
% L(\treelabeling) = & \{ (v, X \cup \treelabeling(v)) \mid (g, \addclass{X}) \in \trs, \\
% & \; v \in \dom(\treelabeling), v, T \models g \}\\
% H(\treelabeling) = & \{ (v.|M_v|, X) \mid (g, \addchild{X}) \in \trs, v \in \dom(\treelabeling),\\
% & |v| < k-1, {v, T \models g}, \forall i \in M_v \, . \, X \not\subseteq {\treelabeling(v.i)} \} 
% \end{align*}
%where $M_v = \makeset{i \mid v.i \in \dom(\treelabeling)}$.
%$\calF (\treelabeling) = \treelabeling \cup \makeset{(v, X \cup \treelabeling(v)) \mid (g, \addclass{X}) \in \trs, v, T \models g} \cup \makeset{(v.|M|, X) \mid (g, \addchild{X}) \in \trs, {v, T \models g}, \forall i \in M \, . \, X \not\subseteq {\treelabeling(v.i)} \text{ where }M = \makeset{i \mid v.i \in \dom(\treelabeling)}}$.

\begin{lemma}\label{lem:fix-property}
\begin{enumerate}[(i)]
\item $T_0 \trleq T_F$.
\item If $T \to_\sigma T'$ then $T' \trleq F(T)$. 
\end{enumerate}
\end{lemma}

\begin{proof}
\begin{inparaenum}[(i)]
\item The witnessing function extends the identity map.
\item Two cases. If $\sigma = (g, \addclass{X})$ then $T' \trleq F(T)$ is witnessed by the identity map. If $\sigma = (g, \addchild{X})$, define the following witnessing function $f_c$ where $f_c \restriction D_\tree$ extends the identity map, and for $v = u.|M_u| \not\in D_\tree$, set
\[
f_{\rm c} (u.|M_u|) := 
\left\{
	\begin{array}{ll}
	u.|M_u| & \hbox{if $\forall i \in M_u . X \not\subseteq \treelabeling_\tree(u.i)$}\\
	u.i_0 & \hbox{if $X \subseteq \treelabeling_\tree(u.i_0)$}
	\end{array}
\right.
\]
\end{inparaenum}
\end{proof}

Take $\tree \in \post_\trs^*(\tree_0)$. Suppose $\tree \trleq \tree_F$. If $\tree \to_\sigma \tree'$ then $\tree' \trleq F(\tree) \trleq F(\tree_F) =_{\rm t} \tree_F$, by Lemmas~\ref{lem:monotone} and \ref{lem:fix-property}. Thus we have the following.
\begin{corollary}[Correctness]
$\tree \trleq \tree_F$ for each $\tree \in \post_\trs^*(\tree_0)$.
\end{corollary}
 


==> lower.tex <==
\section{Lower bounds}
\label{sec:lower}
%\subsection{$\W[1]$-hardness}
In this section, we shall only give a proof of the $\W[1]$-hardness,
leaving the $\PSPACE$ and $\EXP$ lower bounds in the appendix due to
lack of space.

To prove $\W[1]$-hardness, we reduce from the short acceptance problem of
nondeterministic Turing machines.
%: given a triple $\langle \TM,w,k \rangle$,
%where $\TM$ is an NTM, $w \in \{0,1\}^*$ is an input word, and $k$ is positive
%integer represented in unary, decide whether $\TM$ accepts $w$ in $k$
%steps.
The input to the problem is $\langle \TM,w;k\rangle$, where $\TM$ is an NTM,
$w$ is an input word for $\TM$, and $k \in \N$ given in unary.
Suppose that $\TM =
(\oalphabet,\talphabet,\blank,\controls,\pdsrules,q_0,q_{acc})$,
where $\oalphabet = \{0,1\}$ is the input alphabet, $\talphabet =
\{0,1,\blank\}$ is the tape alphabet, $\blank$ is the blank symbol, $\controls$
is the set of control states, $\pdsrules \subseteq (\controls \times \talphabet)
\times (\controls \times \talphabet \times \{L,R\})$ is the transition relation
($L$/$R$ signify go to left/right), $q_0 \in \controls$ is the initial
state, and $q_{acc}$ is the accepting state. Each configuration of $\TM$ on $w$
of length $k$ can be represented as a word
\[
    (0,a_0,c_0)(1,a_1,c_1)\cdots (k,a_k,c_k)
\]
where $a_i \in \talphabet$ for each $i \in [0,k]$, and for some $j \in [0,k]$
we have $c_j \in \controls$ and for all $r \neq j$ it is the case that
$c_j = \star$. Note that this is a word (of a certain kind) over $\Omega := \Omega_k := [0,k] \times \talphabet
\times (\controls \cup \{\star\})$. In the sequel, we denote by
$\CONF_k$ the set of all configurations of $\TM$ of length $k$.
Suppose that $w = a_1\cdots a_n$. If
$n < k$, we append some blank symbols at the end of $w$ and assume that
$|w| \geq k$. The initial configuration will be
$I_0(w) := (0,\blank,q_0)(1,a_1,\star)\cdots (k,a_k,\star)$. [Notice that
if $n > k$, then some part of the inputs will be irrelevant.]
In the following, we will append the symbol $(-1,\blank,\star)$ (resp.
$(k+1,\blank,\star)$) before the start (resp. after the end) of $\TM$
configurations to aid our definitions. Therefore, define
$\Omega_e := \Omega_{k,e} := [-1,k+1] \times \talphabet
\times (\controls \cup \{\star\})$.

%\lo{Why go beyond ${[0, k]}$?}

We now construct a tree-rewrite system $\pds$ to simulate $\TM$.
First off,
for each $\pdsrules$-rule $\sigma$,
define a relation $R_\sigma \subseteq \Omega_e^4$ such that
$(\vecV_1,\vecV_2,\vecV_3,
\vecW) \in R$ iff a configuration $C_2 = \vecU_{-1} \cdots
\vecU_{k+1}$ of $\TM$, where $\vecU_{i+1} = \vecW$ for some $i$, can be
reached in one step using $\sigma$ from another
configuration
$C_1 = \vecU_{-1}' \cdots \vecU_{k+1}'$, where $\vecU_i'\vecU_{i+1}'\vecU_{i+2}' =
\vecV_1\vecV_2\vecV_3$. Let $R = \bigcup_{\sigma\in\pdsrules} R_\sigma$.
In this case, we say that rule $\sigma$ is a witness
for the tuple $(\vecV_1,\vecV_2,\vecV_3,\vecW)$. Notice that, given a rule
$\sigma$ of $\pds$ and $\vecV_1,\vecV_2,\vecV_3$, there exists
\emph{at most one} $\vecW$ such that $(\vecV_1,\vecV_2,\vecV_3,\vecW)
\in R$ and is witnessed by $\sigma$. In addition,
it is easy to see that checking whether
$(\vecV_1,\vecV_2,\vecV_3,\vecW) \in R$ can be done in polynomial time
(independent of $k$) since this is a simple local check of $\TM$
rules.

The rewrite system $\pds$ works over trees of labels $\Xi = \Omega_e
\cup \pdsrules$.
%\lo{As defined, labels must be elements of a power set $\treelabels = 2^\CLASS$.}
The initial tree is a tree with a single node labeled by
$I_0(w)$. We add the following rules to $\pds$:
\begin{enumerate}
\item For each $\sigma \in \pdsrules$, we add $(\top,\addchild{\sigma})$
    to $\pds$.
\item For each $(\vecV_{i-1},\vecV_i,\vecV_{i+1},\vecW) \in R$ witnessed by
    $\sigma \in \pdsrules$, for $i \in [0,k]$,
    we add $(\sigma \wedge \langle \uparrow
    \rangle\{\vecV_{i-1},\vecV_i,\vecV_{i+1}\},
    \addclass{\vecW})$ to $\pds$.
\item For each $\sigma \in \pdsrules$, we add
    $(\sigma,\addclass{(-1,\blank,\star)})$ and
    $(\sigma,\addclass{(k+1,\blank,\star)})$ to
    $\pds$.
\end{enumerate}
Rule 1 first guesses the rule $\sigma$ to be applied to obtain the next
configuration $C_2$ of the NTM $\TM$. This rule is added as a class in the
child $v$ of the current node $u$ containing the current configuration $C_1$.
Rule 3 is then applied to obtain the left and right delimiter. After that,
configuration $C_2$ is written down in node $v$ by applying Rule 2 for $k$
times. In particular, the system will look up the rule $\sigma$ that was
guessed before and the content of the parent node $u$ (i.e. $C_1$). If we
let $S = [0,k] \times \talphabet \times \{q_{acc}\}$, then $S$ is not
$k$-redundant iff $\TM$ accepts $w$ within $k$ steps. Notice that this is
an fpt-preserving reduction. In particular, it runs in time $O(k^c n^d)$
for some constant $c$ and $d$.

%\subsection{$\PSPACE$-hardness}


==> preliminaries.tex <==
% !TEX root = main-LICS14.tex
\section{Preliminaries}
\label{sec:preliminaries}

\al{Maybe this section can be removed. Some stuff can be relegated to the
other sections or appendix.}
\OMIT{
\subsection{Trees}
In this paper we use unordered unranked trees. A
\defn{tree domain} is a subset $\treedomain$ of $\N^*$ (where $\N = \{0, 1, \cdots \}$) that satisfies: % the following properties:
%\begin{inparaenum}[(i)]
%\item
prefix-closure, i.e., $w.i \in \treedomain$ %and $i \in \N$
implies $w \in \treedomain$. %\al{I just removed closure under sibling ordering
%since this only obfuscates our notation.}
%\item closure under sibling ordering, i.e.,
%$w.(i+1) \in \treedomain$ %and $i \in \N$
%implies $w.i \in \treedomain$.
%\end{inparaenum}
%\alchanged{In the sequel, for $v,v' \in \N^*$, we say that $v'$ is a successor
%of $v$
%(written $v \succ v'$) if $v' = v.i$ for some $i \in \N$. We denote by
%$\leq$ the transitive-reflexive closure of $\succ$. Note that $\leq$ is the
%prefix-of relation.}
For $v, v' \in \N^*$, we write $v \leq v'$ to mean that $v$ is a prefix of $v'$.

An \defn{(unordered) tree} over the nonempty finite set (a.k.a. alphabet)
$\treelabels$ is a logical
structure of the form $\tree =
(\treedomain,\treelabeling,\leq)$ where $\treedomain$ is a tree domain and
$\treelabeling$ is a mapping (a.k.a. \defn{node labeling}) from $\treedomain$
to $\treelabels$. As usual in logic, we do not distinguish isomorphic trees,
i.e., trees that are identical after renaming of nodes in $\treedomain$. In the
sequel, when describing $\tree$ we shall omit mention of the relation $\leq$
and simply
write $\tree = (\treedomain,\treelabeling)$. We use standard terminologies for
trees, e.g., parents,
children, ancestors, descendants, and siblings. The \defn{level of a node $v
\in\treedomain$} in $\tree$ is $|v|$. Likewise, the \defn{height
of the tree $\tree$} is $\max\{|v| : v \in \treedomain\}+1$.
Set $\trees(\treelabels)$ to be the set of %all
trees over $\treelabels$. For every $k \in \N$, we define
$\trees_k(\treelabels)$ to be the set of trees of height $k$.

If $\tree = (\treedomain,\treelabeling)$ and $v \in \treedomain$,
the \defn{subtree of $\tree$ rooted at $v$} is the tree
$\tree_{\mid_v} = (\treedomain',\treelabeling')$, where
$\treedomain' := \{ w \in \N^* : vw \in \treedomain \}$ and
$\treelabeling'(w) := \treelabeling(vw)$.

\OMIT{
An \defn{unordered tree} over the alphabet
$\treelabels$ is an ordered tree $\tree$ over $\treelabels$ where
we forget the sibling ordering. Formally we may define an equivalence
relation $\sim$ between ordered trees as follows: $\tree \sim
\tree'$ iff $\tree'$ can be obtained from $\tree$ by finitely many applications
of node-swapping operations between two sibling nodes.
An unordered tree can then be defined as any equivalence class in
$\trees(\treelabels)/\sim$.
}

\mh{removed term representation of trees since afaik we don't use it.}


\OMIT{
\subsection{Pushdown systems}
A \defn{pushdown system (PDS)} is a tuple $\pds =
(\controls,\salphabet,\pdsrules)$, where
$\controls$ is a finite set of \defn{control states}, $\salphabet$ is a finite
set of \defn{stack symbols},
and $\pdsrules$ is a finite subset of $(\controls \times \salphabet) \times
(\controls \times \salphabet^*)$ such that if $((q,a),(q',w)) \in \pdsrules$
then $|w| \leq 2$. This PDS generates a transition relation $\to_\pds
\subseteq (\controls \times \salphabet^*) \times (\controls \times \salphabet)$
as follows: $(q,v) \to_\pds (q',v')$ if there exists a rule
$((q,a),(q',w)) \in \pdsrules$ such that $v = ua$ and $v' = uw$ for some
word $u \in \salphabet^*$.
}

\subsection{Complexity classes}
We assume standard concepts from computational complexity: $\P$, $\PSPACE$,
$\EXP$. We also use some standard concepts from parameterized complexity
theory (see \cite{grohe-book} for a thorough treatment).

A \defn{parameterized
problem} $\mathcal{C}$ is a computational problem with input of the form
$\langle v;k\rangle$,
where $v \in \{0,1\}^*$ and $k \in \N$ (represented in unary) is called the
\emph{parameter}.
An \defn{fpt-algorithm} for $\mathcal{C}$ runs in time $O(f(k) . n^c)$ for
some constant $c$, and some computable function
$f: \N \to \N$ (both independent of input). Here, $n$ is the size of the input.
So, an algorithm that
runs in time $O(n^k)$ is not an fpt-algorithm. The problem $\mathcal{C}$
is said to be \defn{fixed-parameter tractable} if it can be solved by an
fpt-algorithm. There are classes of problems in parameterized complexity
that are widely believed not to be solvable by fpt-algorithms, e.g.,
$\W[1]$ (and others in the $\W$-hierarchy). To show that a problem
$\mathcal{C}$ is $\W[1]$-hard, it suffices to give an fpt-reduction
to $\mathcal{C}$ from the \defn{short acceptance problem of nondeterministic
Turing machines (NTM)}: given a tuple $\langle (\TM,w);k \rangle$,
where $\TM$ is an NTM, $w \in \{0,1\}^*$ is an input word, and $k$ is a positive
integer represented in unary, decide whether $\TM$ accepts $w$ in $k$
steps. Among others, standard reductions in complexity theory that satisfy the
following two conditions are fpt-reductions: (1) fpt-algorithms, (2) if
$k$ is the input parameter, then the output parameter is $O(k)$.
\OMIT{
The set of $k$-fold exponential functions is defined inductively.
A $0$-fold exponential function is any polynomial function $f: \N \to \N$; for
each $k \in \N_{> 0}$, a $k$-fold exponential function is any function of the
form $2^{f(n)}$, where $f$ is any $(k-1)$-fold exponential function.
We use $k$-$\EXPSPACE$ to mean the set of problems solvable by Turing
machines equipped with $k$-fold exponential bounded space.
}



==> relatedwork.tex <==
% !TEX root = main.tex

\section{Related Work}




==> restriction.tex <==
% !TEX root = main.tex
\section{Restriction}
\label{sec:restrict}

This section studies a restriction of the rewrite systems with better
complexity. Let us call a guard $g$ \defn{upward-looking} if it has \emph{no}
occurrence of $\langle \downarrow \rangle$. Using such guards, a node can only
inspect the values of its ancestors. In this section, we will look at the
subclass $\utrsclass$ of $\trsclass$ where all rewrite rules have only
upward-looking guards. Likewise, for the redundancy and $k$-redundancy problems
for $\utrsclass$, we assume that the guard database has only upward-looking
guards.


\begin{theorem}
The redundancy problem for $\utrsclass$ is $\PSPACE$-complete.
\end{theorem}
\begin{proof}

\textbf{Upper Bound.} \lo{For the case with $\addchild{-}$ only, the upper bound is $\PSPACE$; in general, the best known upper bound is $\EXP$.}

We now establish a nondeterministic algorithm that solves the problem in polynomial space. The input to the problem is a rewrite system $\trs$, an initial tree $\tree_0$, and a set $S$ of guards. Let $k$ be the maximum $\langle \uparrow \rangle$-nesting depth of guards in $S$.
\smallskip

\noindent
\textbf{Lower Bound.} To show $\PSPACE$-hardness, we give a reduction from
membership for a fixed linear bounded Turing machines
$M = (\oalphabet,\talphabet,\blank,\controls,\pdsrules,q_0,q_{acc})$,
where $\oalphabet = \{0,1\}$ is an input alphabet, $\talphabet =
\{0,1,\blank\}$ is the tape alphabet, $\blank$ is the blank symbol, $\controls$
is the set of control states, $\pdsrules: (\controls \times \talphabet)
\to (\controls \times \talphabet \times \{L,R\})$ is the transition function
($L$/$R$ signify go to left/right), $q_0 \in \controls$ is the initial
state, and $q_{acc}$ is the accepting state. Given an input word $w \in
\oalphabet^*$, each configuration of $M$ has length precisely $l(n)$, for $n =
|w|$ and some linear function $l: \N \to \N$. Hence, the initial configuration
is $I_0(w) = (q_0,\blank)a_1\cdots a_n\blank^{l'(n)}$, where $l'(n) =
l(n) - n - 1$.

The reduction works as follows. The output rewrite system works over the
alphabet $\treelabels := \{\#\} \cup (Q \times \talphabet) \cup \talphabet$.
The initial tree $\tree_0$ is $\#I_0(w)$. The rewrite rules are as follows:
\begin{enumerate}
\item for each $a \in \treelabels$, add $( (a\langle \uparrow \rangle)^{l(n)}
    \#, \addchild{\#} )$.
\item for each $a,b,c \in \treelabels$,
    \begin{itemize}
    \item if $a,b,c \notin (Q \times \talphabet)$, then add
    \[
        ( \langle \uparrow \rangle^{l(n)-1}c\langle \uparrow \rangle b
        \langle \uparrow \rangle a,
        \addchild{b} ).
    \]
    \item if $a = (q,i)$ and $\pdsrules(q,i) = (q',i',L)$, then add
    \[
        ( \langle \uparrow \rangle^{l(n)-1}c\langle \uparrow \rangle b
        \langle \uparrow \rangle a,
        \addchild{b} ).
    \]
    \item if $a = (q,i)$ and $\pdsrules(q,i) = (q',i',R)$, then add
    \[
        ( \langle \uparrow \rangle^{l(n)-1}c\langle \uparrow \rangle b
        \langle \uparrow \rangle a,
        \addchild{(q',b)} ).
    \]
    \item if $b = (q,i)$ and $\pdsrules(q,i) = (q',i',d)$ for
        some $d \in
        \{L,R\}$, then add
    \[
        ( \langle \uparrow \rangle^{l(n)-1}c\langle \uparrow \rangle b
        \langle \uparrow \rangle a,
        \addchild{i'} ).
    \]
    \item if $c = (q,i)$ and $\pdsrules(q,i) = (q',i',R)$, then add
    \[
        ( \langle \uparrow \rangle^{l(n)-1}c\langle \uparrow \rangle b
        \langle \uparrow \rangle a,
        \addchild{b} ).
    \]
    \item if $c = (q,i)$ and $\pdsrules(q,i) = (q',i',L)$, then add
    \[
        ( \langle \uparrow \rangle^{l(n)-1}c\langle \uparrow \rangle b
        \langle \uparrow \rangle a,
        \addchild{(q',b)} ).
    \]
    \end{itemize}
\end{enumerate}
Notice that in general the rewrite system $\trs$ outputs \emph{trees}
possibly with multiple branches. However, since $M$ is deterministic, for two
branches (i.e. words) $B_1, B_2$ produced by $\trs$, either $B_1 \leq B_2$
or $B_2 \leq B_1$. It is easy to see now that $M$ accepts the input word $w$
iff $(q_{acc},\blank)$ is not redundant. \qed
\end{proof}



\begin{theorem}
\begin{enumerate}[(i)]
\item The redundancy problem for $\usstrsclass$ with $\addchild{-}$ only is $\PSPACE$-complete.
\item The redundancy problem for $\usstrsclass$ is decidable in $\NEXP$ and $\PSPACE$-hard.
\end{enumerate}
\end{theorem}

\begin{theorem}
\begin{enumerate}[(i)]
\item The redundancy problem for $\ustrsclass$ with $\addchild{-}$ only is $\NP$-complete.
\item The redundancy problem for $\ustrsclass$ is $\NP$-hard.
\end{enumerate}
\end{theorem}


\lo{Rough notes: Encoding SAT.

Given an instance $C_1 \wedge \cdots \wedge C_n$. Begin with rules:
\[
\begin{array}{l}
((x_1, i), \addchild{(x_2, j)})\\
((x_2, i), \addchild{(x_3, j)})\\
\qquad \vdots\\
((x_{n-1}, i), \addchild{(x_n, j)})\\
%((x_n, i), \addchild{\, C_1)
\end{array}
\]
where $i, j \in \{0,1\}$.

Suppose $C_1 = x_{1} \vee x_{2} \vee \neg x_{5}$. Then add rules:
\[\begin{array}{l}
(\uparrow^+  (x_{1}, 1), \addchild{C_1})\\
(\uparrow^+  (x_{2}, 1), \addchild{C_1})\\
(\uparrow^+  (x_{5}, 0), \addchild{C_1})
\end{array}\]

Similarly for $C_2, \cdots, C_n$.

Finally
\[
(\uparrow^+ C_n \, \uparrow^+ C_{n-1} \cdots \uparrow^+ C_1, \addchild{F})
\]
}

\begin{theorem}
The $k$-redundancy problem for $\utrsclass$ is $\NL$-complete.
\end{theorem}
\begin{proof}
To show $\NL$-hardness, we can establish a logspace reduction from graph
reachability (of directed graphs) to the $k$-redundancy problem for
$\utrsclass$. In fact, in this case, it suffices to restrict ourselves to
rewrite rules of the form $\changecolor{a}$.

The reduction works as follows. Suppose that we are given a graph $G = (V,E)$,
a source node $s \in V$, and a sink node $t \in V$.
The output rewrite system $\trs$ works over the set $\treelabels = V$
of node labeling. For each edge $(u,v) \in E$, we output a rewrite rule of the
form $(\langle u \rangle,\changecolor{v})$.  It is easy to see that $s \to_G^*
t$ iff the guard $\langle v\rangle$ is redundant for $\trs$ when started with
the initial tree $\tree_0 = s$. Finally, it is easy to see that this
can be implemented in logspace. \qed
\end{proof}

